Direct Prediction of 3D Body Poses from Motion Compensated Sequences

We propose an efficient approach to exploiting motion information from consecutive frames of a video sequence to recover the 3D pose of people. Previous approaches typically compute candidate poses in individual frames and then link them in a post-processing step to resolve ambiguities. By contrast, we directly regress from a spatio-temporal volume of bounding boxes to a 3D pose in the central frame. We further show that, for this approach to achieve its full potential, it is essential to compensate for the motion in consecutive frames so that the subject remains centered. This then allows us to effectively overcome ambiguities and improve upon the state-of-the-art by a large margin on the Human3.6m, HumanEva, and KTH Multiview Football 3D human pose estimation benchmarks.

==> tmp.tex <==
%% -*- mode: latex; mode: reftex; mode: flyspell; mode: auto-fill; TeX-master: "top.tex"; -*-
\subsection{Implementation Details}

We collect  every block of $T=24$ consecutive frames to compute 3D HoG feature across
all   training   videos. The influence of the length of temporal
window is show in Section \ref{XXX}. We pick $24$ considering the
balance of performance and speed. 
Our multi-scale 3D HoG feature uses 3 level by  dividing the
spatial dimensions into $2  \times 2$, $4 \times 4$ and $8  \times 8$
cells. The temporal bin  size of 3D HOG  is set to a  small value, $4$ frames  for $50$ fps
videos,  to  model   subtle  changes  in  the  motion.   

As done like other approaches, we use 17 joints for Huam36m dataset,
xx joints for HumanEva dataset.

We use kernel ridge regression (KRR) and kernel dependency estimation (KDE) to learn 
the model for our regressor. For KRR and KDE, an input kernel embedding of 15,000 dimensional random 
feature maps corresponding to exponentiated $\chi^2$ and a 4000-dimensional
output embedding corresponding to radial basis function kernel  is
used. We learn the regressor for each action individually. We also
report a general motion regressor which is trained from all the
actions in Human36 dataset, which has simliar performance with
individual regressors.
